Enhancing Adversarial Defense by k-Winners-Take-All

We propose a simple change to existing neural network structures for better defending against gradient-based adversarial attacks. Instead of using popular activation functions (such as ReLU), we advocate the use of k-Winners-Take-All (k-WTA) activation, a C0 discontinuous function that purposely invalidates the neural network model's gradient at densely distributed input data points. The proposed k-WTA activation can be readily used in nearly all existing networks and training methods with no significant overhead. Our proposal is theoretically rationalized. We analyze why the discontinuities in k-WTA networks can largely prevent gradient-based search of adversarial examples and why they at the same time remain innocuous to the network training. This understanding is also empirically backed. We test k-WTA activation on various network structures optimized by a training method, be it adversarial training or not. In all cases, the robustness of k-WTA networks outperforms that of traditional networks under white-box attacks.

==> Makefile <==
# name of latex document
MAINDOC := main

# latex source file
TEXSRC := main.tex $(wildcard *.tex)
BIBSRC := $(wildcard *.bib)

ifneq ($(strip $(BIBSRC)),)
BBLSRC := $(MAINDOC).bbl
endif

# latex program
TEX      := latex
PDFLATEX := pdflatex
BIB      := bibtex

# flags
TEX_FLAGS :=
PDF_FLAGS :=
BIB_FLAGS :=

#=====================================================#
# Display Codes (this is so we can track passes)
#=====================================================#
MOVE_TO_COL	= @echo  "\\033[60G"
SETCOLOR_RED 	= @echo  "\\033[0;31m"
SETCOLOR_GREEN 	= @echo  "\\033[0;32m"
SETCOLOR_BLUE	= @echo  "\\033[0;34m"
SETCOLOR_BACK	= @echo  "\\033[0m"

all: $(MAINDOC).pdf

pdf: $(MAINDOC).pdf

dvi: $(MAINDOC).dvi

full: $(BBLSRC) $(TEXSRC)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)
	$(SETCOLOR_GREEN)
	@echo "=========================FINAL PASS=============================="
	$(SETCOLOR_BACK)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)


%.dvi : %.aux
	$(SETCOLOR_BLUE)
	@echo "=========================AUX -> DVI PASS=============================="
	$(SETCOLOR_BACK)
	@$(TEX) $(TEX_FLAGS) $(*F)
	
$(MAINDOC).bbl : $(BIBSRC) $(TEXSRC) 
ifneq ($(strip $(BIBSRC)),)
	$(SETCOLOR_GREEN)
	@echo "=========================LaTeX PASS=============================="
	$(SETCOLOR_BACK)
	$(PDFLATEX) $(TEX_FLAGS) $(MAINDOC)
	$(SETCOLOR_GREEN)
	@echo "=========================BibTex PASS=============================="
	$(SETCOLOR_BACK)
	@$(BIB) $(BIB_FLAGS) $(MAINDOC)
endif

$(MAINDOC).pdf : $(TEXSRC)
	$(SETCOLOR_GREEN)
	@echo "=========================SINGLE PASS=============================="
	$(SETCOLOR_BACK)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)

.PHONY: all clean

clean:
	-$(RM) *.aux *.pdf *.bbl *.blg *.log


==> exp2_old.tex <==
\section{Additional Experimental Results}

\subsection{Efficacy of Incremental Training}
\begin{figure*}[t]
	\centering
	%\vspace{-1mm}
	\includegraphics[width=1.0\textwidth]{figs/ft.pdf}
	\vspace{-5mm}
	\caption{
            \textbf{Efficacy of incremental training.} We sweep through a 
            range of sparsity ratios, and evaluate the standard and robust accuracies
            of two network structures (left: ResNet18 and right: Wide ResNet).
            We compare the performance differences between the regular training (i.e.,
            training without incremental fine-tuning) and the training
            with incremental fine-tuning.
	}
    \label{fig:ft}
	\vspace{-3mm}
\end{figure*}

First, we demonstrate the efficacy of incremental training (described
in \secref{train}).  
As shown in \figref{ft}, models trained with incremental fine-tuning (denoted
as \textsf{w/ FT} in the plots' legend) performs better in terms of both standard
accuracy (denoted as \textsf{std} in the plots' legend) and robust accuracy (denoted
as \textsf{rob} in the plots) when $\gamma<0.2$,  suggesting that 
fine-tuning is worthwhile when $\gamma$ is small.

\subsection{Complete Results on PGD attack}\label{sec:gdattack2}
In \tabref{cifar_main2},
we report the detailed robustness results for different architectures and
attack configurations on CIFAR dataset.
The adversarial examples used for \emph{attack tests} are constructed by PGD ( for 20
iterations with random initialization).  The step size of the PGD attack is
$\epsilon/10$, where $\epsilon$ is the perturbation size.  
We experimented with different $\epsilon$ values as shown in \tabref{cifar_main2}

On the other side, the adversarial examples used for
\emph{adversarial training} are also constructed by PGD (for 20 iterations with random
initialization), with the maximum perturbation range $\epsilon=8$ (or 0.031 after
normalizing pixel values into [0, 1]) 
under $\ell_{\infty}$-norm and a step size of 0.003. 
All the input images are normalized into [0, 1] before fed into the network.

We find that, after optimized using adversarial training, 
\kwta models generally outperform ReLU models that are also optimized with adversarial training.
In addition, a wider network (DenseNet, Wide ResNet)
performs better than a narrower one---a finding that validates our theoretical analysis in \secref{theory}:
recall that \thmref{dense} states that increasing network width can improve the robustness
of \kwta models.
\begin{table}[t]
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l|l|cccccc}
% \hline \hline
\bottomrule
Activation & Model & $\epsilon=0$ ($A_{std}$) & $\epsilon=1$ & $\epsilon=2$ &$\epsilon=4$ & $\epsilon=8$     \\ \hline 
ReLU & ResNet18  &  90.9\%  & 27.2\%   & 5.7\%  & 0.1\%  &  0.00\%   &          \\
ReLU & ResNet18+adv        &  83.1\%  &  79.5\%  & 74.6\% & 65.8\% &  42.9\% &           \\
ReLU& ResNet18+TRADE      & 78.9\%    & 76.2\%   & 71.9\% & 65.8\% &  50.1\%  &           \\ 

\kwta & ResNet18-0.08        &  85.8\%  & 67.0\%   & 51.3\% & 30.7\% &  17.7\%   &           \\
\kwta & ResNet18-0.08+adv    &  73.3\%  & 70.7\%    & 68.1\% & 63.2\% & \textbf{ 52.4\%}  &           \\
\kwta & ResNet18-0.08+TRADE  &  70.0\%  & 68.0\%   & 65.2\% & 61.5\% &  51.0\%  &           \\
ReLU & DenseNet121 & 91.1\%   &13.3\%    & 1.5\%  & 0.0\%  & 0.0\%    &           \\
ReLU & DenseNet121+adv     & 84.2\%   &80.0\%    & 75.3\% & 66.8\% & 46.1\%   &           \\
\kwta & DenseNet121-0.09     & 89.5\%   &76.9\%    & 58.5\% & 30.3\% & 8.8\%   &           \\
\kwta & DenseNet121-0.09+adv & 79.3\%   & 77.2\%  & 76.7\%  &73.9\%  & \textbf{66.2\%}  &     \\
ReLU & WideResNet & 91.0\% & 10.1\%   & 0.8\%  &   0.0\%&     0.0\%&     \\
ReLU & WideResNet+adv      &  83.3\%  &  80.0\%  & 75.6\% & 66.2\% &  43.1\%    &     \\
\kwta & WideResNet-0.1      & 88.6\%   & 74.6\%   & 57.7\% & 36.0\% &  22.5\%  &     \\
\kwta& WideResNet-0.1+adv  & 73.8\%   & 71.4\%    & 70.0\% & 66.8\% & \textbf{59.3\%}    &     \\
% \hline \hline
\toprule
\end{tabular}
}
\caption{Results on CIFAR for different perturbation size $\epsilon$.
[Model Name]-0.1 denotes $k$-WTA model trained with sparsity $\gamma=0.1$;
+adv denotes model trained with adversarial training;
+TRADE denotes model trained with TRADE.
}\label{tab:cifar_main2}
\vspace{-3mm}
\end{table}

\subsection{Other Gradient-Based Attack}\label{sec:othergd}
In addition to PGD tests,
we also evaluate our method against various other gradient-based attack methods. 
Our tested attacks include C\&W ($\ell_2$)~\cite{carlini2017towards} attack,
Momentum attack~\cite{dong2018boosting} and Deepfool~\cite{moosavi2016deepfool}.
We use Foolbox~\cite{rauber2017foolbox}, a third-party toolbox for evaluating
adversarial robustness. 

In different attack methods, we have the following setups for generating adversarial examples:
For C\&W ($\ell_2$) attack, we set the binary search step to 5, maximum number of iterations to 20, 
learning rate to 0.01,
and initial constant to 0.01.
For Deepfool, we use 20 steps and 10 sub-samples in its configuration.
For momentum attack, we set the step size to 0.007 and number of iterations to 20.
All other parameters are set by Foolbox to be its default values.

In all attack methods, we use 2000 adversarial samples to evaluate the robust accuracy of each
model.  The results on CIFAR and SVHN are listed in \tabref{cifar_other} and
\tabref{svhn_other}, respectively. The perturbation range of all adversarial samples 
are clipped into the range [-0.031, 0.031] on CIFAR and the range [-0.047, 0.047] on SVHN 
(while the image pixel values are normalized in [0, 1]). 
We also find that in some rare cases, other gradient-based attack methods may produce a slightly
higher rate of successful attacks than PGD on our \kwta model, but 
in general, PGD remains the most effective attack method in our tests.

\subsection{Additional Black-Box Attack Results}\label{sec:black}
\paragraph{Transfer attack.}
We now present the detailed results under transfer attacks in black-box setting on
CIFAR (see \tabref{cifar_transfer}) and SVHN (see \tabref{svhn_transfer}).  
We find that in many transfer attack settings, 
adversarially trained \kwta models does not produce better results in
comparison to adversarially trained ReLU models.  We believe that this is
mainly because that \kwta models with adversarial training usually have
slightly lower standard accuracies than ReLU models.  
% This suggests that \kwta model with adversarial training may not be an ideal
% defense when only consider the black-box attack threat model.  Besides, 
We also find that the particular model, \kwta+DenseNet121-0.09+adv, 
has its robust accuracy under transfer attack lower than 
white-box gradient-based attack.
While not a general phenomenon,
it seems to suggest for this particular model black-box transfer attack 
is more effective than white-box gradient-based attack.
%  robust accuracy on transfer attack
%  is even lower than on gradient-based attack. 
% This is possible due to the
% obfuscated gradient lead to an ineffective gradient-based attack, 
This is possible because our method is particularly motivated for defensing against 
gradient-based attacks.
Similar phenomena have been discussed for previous gradient-based defense methods
(as pointed out in~\cite{obfuscated-gradients}).
In general, the most effective is still the gradient-based attack. 

\begin{table}[t]
\centering
% \resizebox{0.8\columnwidth}{!}{
\begin{tabular}{l|l|ccccc}
% \hline \hline
\bottomrule
Activation & Model & $A_{std}$ & Momentum & Deepfool &  C\&W &     \\ \hline
ReLU & ResNet18   &  88.9\%  & 0.5\%   & 1.0\%  & 0.6\%  &            \\
ReLU & ResNet18+adv        &  83.1\%  &  54.3\%  & 45.5\% &  54.7\% &             \\
\kwta & ResNet18-0.08        &  86.1\%  & 32.1\%   & 83.5\% & 37.5\% &            \\
\kwta & ResNet18-0.08+adv    &  73.3\%  & 53.2\%    & 72.4\% & 58.7\% &            \\
\kwta & ResNet18-0.08+TRADE  &  70.0\%  & 55.4\%   & 72.4\% & 60.7\% &           \\
ReLU & DenseNet121 & 90.1\%   & 0.2\%    & 0.6\%  & 1.0\%  &            \\
ReLU & DenseNet121+adv     & 84.2\%   & 52.9\%    & 48.9\% & 58.8\% &           \\
\kwta & DenseNet121-0.09     & 89.6\%   & 26.2\%    & \textbf{88.2\%} & 33.4\% &           \\
\kwta & DenseNet121-0.09+adv & 79.2\%   & \textbf{65.2\%}   & 78.2\% & \textbf{65.1\%}  &      \\
ReLU & WideResNet & 91.1\% & 0.1\%   & 0.8\%  &   0.1\%&         \\
ReLU & WideResNet+adv      &  83.3\%  &  50.0\%  & 49.5\% & 56.2\% &      \\
\kwta& WideResNet-0.1      & 88.7\%   & 34.1\%   & 85.70\% & 32.3\% &       \\
\kwta& WideResNet-0.1+adv  & 73.8\%   & 56.8\%    & 71.2\% & 57.5\% &      \\
\toprule
% \hline \hline
\end{tabular}
% }
\caption{Other gradient-based attack on CIFAR.
}\label{tab:cifar_other}
\vspace{-6mm}
\end{table}

\begin{table}[t]
\centering
% \resizebox{0.8\columnwidth}{!}{
\begin{tabular}{l|ccccc}
% \hline \hline
\bottomrule
Model & $A_{std}$ & Momentum & Deepfool &  C\&W &     \\ \hline 
ResNet18 (Vanilla)  &  88.9\%  & 0.5\%   & 1.0\%  & 0.6\%  &            \\
ResNet18+adv        &  83.1\%  &  54.3\%  & 45.5\% &  54.7\% &             \\
ResNet18-0.08        &  86.1\%  & 32.1\%   & \textbf{83.5\%} & 37.5\% &            \\
ResNet18-0.08+adv    &  80.7\%  & \textbf{71.5\%}    & 82.3\% & \textbf{75.9\%}  &            \\

% \hline \hline
\toprule
\end{tabular}
% }
\caption{Other gradient-based attack on SVHN
}\label{tab:svhn_other}
\vspace{-4mm}
\end{table}



\begin{table}[t]
\centering
% \resizebox{0.8\textwidth}{!}{

\begin{tabular}{l|cc|c}\bottomrule
\backslashbox{Target Model}{Source Model} &  ReLU+ResNet18 &  ReLU+ResNet18+adv  & $A_{std}$
\\ \hline 
ReLU+ResNet18  & 5.9\%& 58.4\% & 90.9\% \\
ReLU+ResNet18+adv  & 71.9\%& 54.1\% & 73.3\% \\
\kwta+ResNet18-0.18 & 41.9\% & 66.3\% & 90.6\%\\ 
\kwta+ResNet18-0.13 & 45.6\% & 66.0\% & 89.7\%    \\  
\kwta+ResNet18-0.08 & 50.1\%  & 62.0\%  & 86.1\%  \\
\kwta+ResNet18-0.08+adv & 50.1\% & 62.0\%  & 86.1\%  \\\hline
ReLU+DenseNet121  & 6.6\%  & 64.8\% & 91.1\% \\ 
ReLU+DenseNet121+adv  & 81.5\%  & 64.8\% & 81.5\% \\ 
\kwta+DenseNet121-0.18 & 26.5\% &71.7\% & 92.6\% \\
\kwta+DenseNet121-0.13 & 32.1\% &70.7\% & 91.7\% \\
\kwta+DenseNet121-0.09 & 37.3\% &67.3\% & 89.5\% \\
\kwta+DenseNet121-0.09+adv & 76.9\% &58.3\% & 79.2\% \\ \toprule
\end{tabular}

% }
\caption{Black-box transfer attack results on CIFAR.
}\label{tab:cifar_transfer}
\vspace{-4mm}
\end{table}

\begin{table}[t]
\centering
% \resizebox{0.8\textwidth}{!}{

\begin{tabular}{l|cc|c}\bottomrule
\backslashbox{Target Model}{Source Model} &  ReLU+ResNet18 &  ReLU+ResNet18+adv  & $A_{std}$
\\ \hline 
ReLU+ResNet18  & 8.9\%& 59.2\% & 92.9\% \\
ReLU+ResNet18+adv  & 79.3\%& 77.9\% & 83.7\% \\
ReLU+ResNet18+TRADE  & 79.3\%& 78.5\% & 86.2\% \\
\kwta+ResNet18-0.2 & 13.5\% & 78.6\% & 92.3\%\\ 
\kwta+ResNet18-0.1 & 42.4\% & 75.8\% & 89.2\%    \\  
\kwta+ResNet18-0.07 & 38.8\%  & 76.4\%  & 88.2\%  \\
\kwta+ResNet18-0.03 & 49.9\% & 71.2\%  & 83.5\%  \\
\kwta+ResNet18-0.1+adv & 73.3\% & 73.4\%  & 82.8\%  \\
\toprule
\end{tabular}

% }
\caption{Black-box transfer attack results on SVHN.
}\label{tab:svhn_transfer}
\end{table}


\paragraph{Boundary attack.}
We use the implementation in Foolbox~\cite{rauber2017foolbox} to generate
adversarial samples from Boundary Attack++~\cite{chen2019boundary}. 
We set the maximum number of evaluations to 1000 while keeping other parameters
as their default values.
Since the query-based black-box attack is extremely slow, we use only 1000
samples to evaluate the accuracy of each model.  

In addition, Athalye et al.~\cite{obfuscated-gradients} argued that 
obfuscated gradient defense may
result in adversarial samples that can be more easily found by brute-force
random search. Therefore, we also test our method against random Gaussian noise
attack.  
All attack are restricted in $\ell_{\infty}$-norm with
a perturbation size $\epsilon=8$ (while the image pixel values are in [0, 255]). 
In the random noise attack,
we use $10^3$ random samples on each test examples.  As reported in
\tabref{blackbox}, random noise attack is not able to find adversarial examples
on either regular models or $k$-WTA models.

From our experiments, we find that Boundary Attack++ can effectively
reduce the accuracy of a regular ReLU model. 
But replacing ReLU with $k$-WTA, even without the expensive adversarial training, 
significantly improves the robust accuracy,
from 19.7\% to 66.20\% as shown in \tabref{blackbox}.  
Here $k$-WTA+adv also has a lower
robust accuracy than ReLU+adv, mainly because $k$-WTA+adv in this case has 
a lower standard accuracy.

\begin{table}[t]
\centering
% \resizebox{0.7\textwidth}{!}{

\begin{tabular}{l|cc}\bottomrule
\backslashbox{Defense Model}{Attack Method}& Gaussian Noise   & Boundary++  
\\ \hline
ResNet18 (Vanilla) & 88.90\%     &  19.70\% \\
ResNet18+adv &       83.12\%    &73.31\%      \\
ResNet18-0.08 &     85.85\%     &66.20\%     \\
ResNet18-0.08+adv &  73.30\%      & 67.73\%         \\ \toprule
\end{tabular}
% }
\caption{Gaussian noise and Boundary++ black-box attack.
}\label{tab:blackbox}
\end{table}

\subsection{Empirical Worst-Case Robustness}
In \tabref{worst}, we report the \emph{worst-case} robustness results 
on all attacking scenarios that we experimented with.
Here the worst-case robustness
refers to the lowest robust accuracy under all attacks (including both white-box and black-box attacks) 
we evaluated.  As shown in \tabref{worst}, 
\kwta models with adversarial training always achieves the best performance
in comparison to other adversarially trained models---including models trained 
with TRADE, the state-of-the-art defense method against white-box attacks.

\begin{table}[t]
\centering
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c}\bottomrule
Activation& Model& Dataset& Metric& $A_{std}$ & Worst case $A_{rob}$ & Which attack
\\ \hline 
ReLU & ResNet18+adv & CIFAR & $\ell_{\infty}$(0.031)& 83.1\% & 45.5\% & PGD \\
ReLU & ResNet18+TRADE & CIFAR & $\ell_{\infty}$(0.031)& 78.9\% & 50.1\% & PGD \\
\kwta & ResNet18-0.08+adv & CIFAR & $\ell_{\infty}$(0.031)& 73.3\% & \textbf{52.4\%} & PGD \\
ReLU & DenseNet121+adv & CIFAR & $\ell_{\infty}$(0.031)& 84.2\% & 46.1\% & PGD \\
\kwta & DenseNet121-0.09+adv & CIFAR & $\ell_{\infty}$(0.031)& 79.3\% & \textbf{58.3\%} & Transfer attack \\
ReLU & WideResNet+adv & CIFAR & $\ell_{\infty}$(0.031)& 83.3\% & 43.1\% & PGD \\
\kwta & WideResNet-0.1+adv & CIFAR & $\ell_{\infty}$(0.031)& 73.8\% & \textbf{56.8\%} & Momentum \\ \hline
ReLU & ResNet18+adv & SVHN  & $\ell_{\infty}$(0.047)& 84.2\% & 44.5\% & PGD \\
\kwta & ResNet18-0.08+adv & SVHN  & $\ell_{\infty}$(0.047)& 80.7\% & \textbf{71.5\%} & Momentum \\
\toprule
\end{tabular}
}
\caption{Empirical worst-case performance evaluation.
}\label{tab:worst}
\end{table}

\subsection{Loss Landscape Visualization}\label{sec:surf}
To help understand how the sparsity ratio $\gamma$ affects \kwta's robustness against 
gradient-based attacks,
we visualize the loss landscapes of \kwta networks when different sparsity ratios $\gamma$ are used,
and the plots are shown in \figref{surf}.
The way we produce the visualizations is the same as \figref{loss} in the main text (see description
in \secref{loss_land}).
As we reasoned in \secref{theory}, a larger $\gamma$ tends to smooth the loss surface of the \kwta network 
with respect to the input, while a smaller $\gamma$ renders the loss
surface more discontinuous and ``spiky''.  
In addition, adversarial training tends to reduce the range of the loss values---a 
similar phenomenon in ReLU networks has 
already been reported~\cite{madry2017towards,tramer2017ensemble}---but 
that does not mean that the loss surface becomes smoother; the loss surface remains spiky.
\begin{figure*}[h!]
	\centering
	%\vspace{-1mm}
	\includegraphics[width=1.0\textwidth]{figs/surf.pdf}
	\vspace{-5mm}
	\caption{Visualization of different model with different $\gamma$.
	}
    \label{fig:surf}
	\vspace{-3mm}
\end{figure*}

\subsection{CNN architecture for MNIST}\label{sec:cnn}
Lastly, in \tabref{mnist_cnn},
we summarize the CNN architectures that we used in our MNIST experiments reported 
in \secref{gdattack}.

\begin{table}[t]
\centering
% \resizebox{0.8\columnwidth}{!}{
\begin{tabular}{l|l}
\bottomrule
Layer &  Parameters      \\ \hline 
Input  &  size = $1\times 28 \times 28 $              \\ \hline
Convolution        &  output channels=128, kernel size=3, padding=1, stride=1 \\ \hline
ReLU/\kwta        &  - \\\hline
Convolution        &  output channels=128, kernel size=3, padding=1, stride=2 \\\hline
ReLU/\kwta        &  - \\\hline
Convolution        &  output channels=256, kernel size=3, padding=1, stride=1 \\\hline
ReLU/\kwta        &  - \\\hline
Convolution        &  output channels=256, kernel size=3, padding=1, stride=2 \\\hline
Linear & input size=12544, output size=10000 \\\hline
ReLU/\kwta & - \\\hline
Linear & input size=10000, output size=10 \\\hline
Softmax output & -\\
\toprule
\end{tabular}
% }
\caption{MNIST CNN architecture used in \secref{gdattack}.
}\label{tab:mnist_cnn}
\end{table}

\clearpage


==> experiment_old.tex <==

% \rev{
% We use the notation \textit{[Model name]-[Sparsity]} to represent a network trained with $k$-WTA,
% e.g., ResNet18-0.2 represents to use ResNet18 as the base structure, 
% with a sparsity ratio $\gamma=0.2$ in $k$-WTA activation.
% }

\vspace{-0.07in}
\vspace{-0.5mm}
\section{Experimental Results}\label{sec:exp}
\vspace{-0.07in}
We now evaluate the \kwta network under various types of 
adversarial attacks and compare it with other defense methods.
When reporting statistics, we use 
$A_{rob}$ to indicate the model accuracy under adversarial attacks
applied to the test dataset,
and $A_{std}$ to indicate the accuracy on the clean test data. %%(without attacks).

% In this section, we verify the effectiveness of $k$-WTA by numerical experiments.
% We use the notation 
% $A_{rob}$ to represent the accuracy of the model when applied with adversarial attack
% on the test dataset
% and $A_{std}$ to represent the accuracy when tested on the clean test data.
% For all dataset we used, we normalize the pixel value of input data to $[0, 1]$.


\vspace{-0.05in}
\subsection{Gradient-Based Attack}\label{sec:gdattack}
\vspace{-0.04in}
\vspace{-0.5mm}
% \paragraph{main results.}
We evaluate our method on three datasets, MNIST~\cite{lecun1998gradient}, CIFAR-10~\cite{krizhevsky2009learning} and
SVHN~\cite{netzer2011reading}, since they have been extensively used in previous research
for evaluating adversarial robustness.  

\paraspace
\paragraph{CIFAR-10.}
On CIFAR-10, we use untargeted \textit{Projected Gradient Descent} (PGD) attack~\cite{kurakin2016adversarial} 
(with random initialization for 20 iterations)
to find adversarial examples that perturb 
image pixels (in the range of [0, 255]) within an $\ell_{\infty}$ $\epsilon$-ball.
We test four perturbation ranges,
with $\epsilon=1,2,4,8$ in terms of pixel values.
Before feeding the images to the network, we normalize them into [0, 1]. 

%  we test our algorithm with different perturbation range, i.e.,
%  $\epsilon=1,2,4,8$, with a pixel value range of [0, 255]. We use
%  $\ell_{\infty}$-norm criterion to define the perturbation, e.g., $\epsilon=4$
%  means the maximum difference on a pixel between perturbed image and original
%  image is 4.  the images was normalized to [0, 1] before feed into the network.
%  The robust accuracy are evaluated using untargeted PGD attack with random
%  restarts for 20 iterations.

\begin{table}[t]
\vspace{-2mm}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{llcccccc}
\toprule
Activation & model & $A_{std}$ & $A_{rob}$($\epsilon=1$) & $A_{rob}$($\epsilon=2$) &$A_{rob}$($\epsilon=4$) & $A_{rob}$($\epsilon=8$)     \\ \hline
\multirow{3}{*}{ReLU}& WRN & 91.0\% & 10.1\%   & 0.8\%  &   0.0\%&     0.0\%&     \\
&WRN+adv      &  83.3\%  &  80.0\%  & 75.6\% & 66.2\% &  43.1\%    &     \\
&WRN+TRADE      & 78.9\%    & 76.2\%   & 71.9\% & 65.8\% &  50.1\%  &           \\ \hline
\multirow{2}{*}{\kwta}&WRN-0.1      & 88.6\%   & \textbf{74.6\%}   & 57.7\% & 36.0\% &  22.5\%  &     \\
&WRN-0.1+adv  & 73.8\%   & 71.4\%    & 70.0\% & 66.8\% & \textbf{59.3\%}    &     \\
\bottomrule
\end{tabular}
}
\vspace{0.3mm}
\caption{Wide ResNet(WRN) on CIFAR with different perturbation sizes.
WRN-0.1 indicates WRN model with \kwta activation of sparsity $\gamma=0.1$ (without adversarial training);
+adv indicates models with adversarial training;
+TRADE indicates models trained with TRADE.
}\label{tab:cifar_main}
\vspace{-6mm}
\end{table}

In \tabref{cifar_main},
we report the results on Wide ResNet (WRN)~\cite{zagoruyko2016wide} with
depth 22 and widen factor 10 (WRN-22-10). We compare our method with adversarial
training~\cite{madry2017towards} and TRADE~\cite{zhang2019theoretically}; both
are considered the state-of-the-art defense against white-box gradient-based attacks.  
Here we use the parameter $1/\lambda=6$ in TRADE, a value that leads to the best robustness 
according to their paper. 

The ReLU networks in our tests are trained with stochastic gradient descent (SGD) with
momentum=0.9.  we using a learning rate 0.1 from 1 to 60 epochs, 0.01 during
60-80 epochs and 0.001 during 80-100 epochs.  
\kwta networks, without adversarial training,
are trained incrementally, starting with $\gamma=0.2$ for 60 epochs with SGD
(learning rate=0.1, momentum=0.9) and then decreasing
$\gamma$ by 0.005 every 2 epochs until $\gamma$ reaches the desired value.
When adversarial training is used,
the \kwta networks are trained in the same way as ReLU networks,
without fine-tuning.

As shown in \tabref{cifar_main}, 
when $\epsilon=1$,
WRN-22-10 with \kwta ($\gamma$=0.1) activation,
even without adversarial training,
achieves a robust accuracy ($A_{rob}$) comparable to
the ReLU model optimized with adversarial training.
Meanwhile, ReLU model without adversarial training can be easily attacked by adversarial 
examples. As $\epsilon$ increases, the accuracy $A_{rob}$ of the $k$-WTA model starts to drop.
However, when adversarial training is employed to train the $k$-WTA network, it outperforms the
ReLU networks with both adversarial training and TRADE.

The advantages of \kwta networks consistently retain on other architectures 
(including ResNet~\cite{he2016deep}, DenseNet~\cite{huang2017densely}) and against different
attack methods (e.g., C\&W attack~\cite{carlini2017towards},
Deepfool~\cite{moosavi2016deepfool}).  
Please refer to \appref{gdattack2} and \appref{othergd} for details.

\paraspace
\paragraph{MNIST and SVHN.}
On MNIST and SVHN datasets, we test our model with perturbation size
$\epsilon$=0.3 and $\epsilon$=0.047, respectively, for pixel values ranged 
in [0, 1].  
The robust accuracy are evaluated under PGD attacks with random initialization for 20 
iterations, and the results are summarized in \tabref{mnistsvhn_main} and \appref{gdattack2}.

\begin{table}[t]
\centering
\vspace{-2mm}
\resizebox{0.92\textwidth}{!}{
\begin{tabular}{l|lcc|lcc}
\bottomrule
Activation & MNIST model & $A_{std}$  & $A_{rob}$       & SVHN Model  & $A_{std}$  &  $A_{rob}$ \\ \hline
\multirow{3}{*}{ReLU}&CNN & 99.4\%  & 0.0\%          & ResNet18 &  95.0\%         & 0.0\%     \\
&CNN+adv     &  99.2\%   & 95.0\%         & ResNet18+adv &  84.2\% &  44.5\%  \\  
&CNN+TRADE   &  99.2\%   &  96.0\%               & ResNet18+TRADE &   87.6\%     &  42.4\%         \\ \hline
\multirow{2}{*}{\kwta}&CNN-0.08     &  99.3\%   & 62.2\%         & ResNet18-0.1  &  89.3\% & 12.1\%                  \\
&CNN-0.08+adv &  99.20\%  & \textbf{96.4\%} & ResNet18-0.1+adv & 83.5\% & \textbf{73.4\%}  \\
\toprule
\end{tabular}
}
\vspace{0.3mm}
\caption{Results on MNIST and SVHN datasets.
    +adv indicates models with adversarial training; 
    +TRADE indicates models trained with TRADE
    \label{tab:mnistsvhn_main}}
\vspace{-4.5mm}
\end{table}


When testing on MNIST dataset, we use a 4-layer
convolutional network trained by SGD with a learning rate 0.01 for 20 epochs.
The CNN architecture details are provided in \appref{cnn},  
and the \kwta CNNs in our test are all trained from scratch without incremental fine-tuning.  
On SVHN dataset, we use
standard ResNet18 and the same optimization protocal as what we used on CIFAR.  
Even without adversarial training, the \kwta model 
already performs slightly better than 
the ReLU model. After using adversarial training, the \kwta model 
outperforms considerably the adversarially trained ReLU model. Especially on SVHN dataset,
the accuracy is boosted from 44.5\% to 73.4\%.

% and Resnet18 for our svhn experiment.

% As shown in \tabref{cifar_main} and \tabref{mnistsvhn_main}, 
% our method achieves similar performance as adversarial trained model on robust accuracy when perturbation size is small, without sacrifice standard accuracy too much.
% When combined with adversarial training, our methods outperforms adversarial training applied on a regular network. 
% Notice that our method considerably improves the state-of-the-art on SVHN dataset,
% without downgrading the standard accuracy.

% We also tested our algorithm on other gradient-based attack, e.g., Deepfool~\cite{moosavi2016deepfool},
% C\&W attack~\cite{carlini2017towards} and Momentum attack~\cite{dong2018boosting}. Please refer to \cmt{Appendix X} for details.


\paraspace
\paragraph{Varying sparsity ratio $\gamma$ and model architecture.}
We further evaluate our method on various network architectures with different sparsity ratios $\gamma$.
\figref{gamma_change} shows the standard test accuracies and robust accuracies 
against PGD attacks while $\gamma$ decreases. %% in our fine-tuning process.  
To test against different network architectures,
we apply \kwta to ResNet18, DenseNet121 and Wide ResNet (WRN-22-12).
In each case, starting from $\gamma=0.2$, we decrease $\gamma$ using incremental fine-tuning.
We then evaluate the robust accuracy on CIFAR dataset, 
taking 20-iteration PGD attacks with a perturbation range $\epsilon=8$ for
pixels ranged in [0, 255].

We find that when $\gamma$ is larger than $\sim 0.1$, reducing $\gamma$ 
has little effect on the standard accuracy, but increases the robust accuracy. 
When $\gamma$ is smaller than $\sim 0.1$, reducing $\gamma$ drastically lowers both the standard
and robust accuracies.
The peaks in the $A_{rob}$ curves (\figref{gamma_change}-right) are consistent with our theoretical
understanding: 
\thmref{dense} suggests that when $l$ is fixed, a smaller $\gamma$ 
tends to sparsify the linear region boundaries, 
exposing more gradients to the attacker.
Meanwhile, as also discussed in \secref{theory}, a smaller $\gamma$ leads to a
larger discontinuity jump and thus tends to improve the robustness.

%  But if $\gamma$ is too small, the activated subnetwork for each data 
%  becomes too limited and thus the performance starts to drop.
%  makes the linear regions denser and thus the network becomes more robust.

\begin{figure*}[t]
	\centering
	%\vspace{-1mm}
	\includegraphics[width=0.90\textwidth]{figs/tune.pdf}
	\vspace{-3mm}
	\caption{Robustness changing w.r.t. $\gamma$ on CIFAR. 
    When $\gamma$ decreases, the standard test accuracy (left) starts to drop after a certain point.
    The robust accuracy (right) first increases then decreases.
	}
    \label{fig:gamma_change}
	\vspace{-3mm}
\end{figure*}

\vspace{-0.06in}
\subsection{Black-Box Attack}
\vspace{-0.05in}
% We verify the robustness of our models under black-box attacks. We first train models without using adversarial
% training on the MNIST and CIFAR10 datasets. We use the same network architectures that are specified in the
% beginning of this section, i.e., the CNN architecture in [CW17] and the WRN-34-10 architecture in [ZK16]. We
% denote these models by naturally trained models (Natural). The accuracy of the naturally trained CNN model
% is 99.50% on the MNIST dataset. The accuracy of the naturally trained WRN-34-10 model is 95.29% on the
% CIFAR10 dataset. We also implement the method proposed in [MMS+18] on both datasets. We denote these
% models by Madry’s models (Madry). The accuracy of [MMS+18]’s CNN model is 99.36% on the MNIST
% dataset. The accuracy of [MMS+18]’s WRN-34-10 model is 85.49% on the CIFAR10 dataset
Next, we evaluate the robustness of \kwta models under black-box attacks.
Note that the use of \kwta is motivated for defending against gradient-based attacks;
it is not specifically designed for defending under black-box attacks.
Regardless, we find that $k$-WTA models still have better robust accuracies than ReLU models,
although with adversarial training $k$-WTA models do
not show better performance in comparison to 
adversarially trained ReLU models.
%  This is mainly because $k$-WTA model with adversarial training
%  usually has lower standard accuracy than adversarially trained ReLU model.
However, when both \kwta and ReLU models are trained on clean data without adversarial training, 
\kwta models (such as ResNet18-0.08) defend much better against black-box attacks.
The results are reported in \tabref{transfer}.

So far the most effective black-box attack is transfer
attack~\cite{papernot2017practical, tramer2017ensemble}, based on the
observations that adversarial examples identified in one network are likely 
to fool other networks trained for the same task. 
To evaluate our models, we use ResNet18 trained on clean CIFAR-10 dataset as the
source model to transfer attack our models.
%% evaluate our black box robustness.
As shown in \tabref{transfer}, $k$-WTA models produce better robust accuracies 
than ReLU models under transfer attacks.  
The robustness-accuracy trade-off~\cite{tsipras2018robustness} can be
also seen in the black-box attack scenario: as $\gamma$ is reduced, the
standard accuracy of the \kwta model will decrease but its robust accuracy increases.  
In addition, we find that when $\gamma$ is relatively
large, \kwta models achieve similar (sometimes even better) standard accuracies
than ReLU models, while maintaining better robustness.  This suggests that
\kwta can be a ``free'' replacement of ReLU activation on classification tasks
with no performance cost.

We in addition evaluate black box accuracies under transfer attacks 
using other source and target models.
% it can still be useful under black box scenario since $k$-WTA can be a "free" replacement
% of other activation function.
Besides transfer attacks, we also evaluate our method on the state-of-the-art
decision-based black box attacks, namely Boundary Attack++~\cite{chen2019boundary}.  
In these experiments, \kwta models achieve considerably better robustness 
against decision-based attacks in comparison to conventional ReLU models. 
We report the result details in \appref{black}.

% \begin{table}[h]
% \centering
% \resizebox{0.8\textwidth}{!}{

% \begin{tabular}{l|cc|c}\hline\hline
% \backslashbox{Target Model}{Source Model} &  ResNet18 (Vanilla) &  ResNet18+adv  & $A_{std}$
% \\ \hline \hline
% ResNet18 (Vanilla) & 5.9\%& 58.4\% & 90.9\% \\\hline
% ResNet18-0.18 & 41.9\% & 66.3\% & 90.6\%\\  \hline
% ResNet18-0.13 & 45.6\% & 66.0\% & 89.7\%    \\  \hline
% ResNet18-0.08 & \textbf{50.1\%}  & 62.0\%  & 86.1\%  \\\hline
% DenseNet121 (Vanilla)  & 6.6\%  & 64.8\% & 91.1\% \\ \hline
% DenseNet121-0.18 & 26.5\% &71.7\% & \textbf{92.6\%} \\\hline
% DenseNet121-0.13 & 32.1\% &70.7\% & 91.7\% \\\hline
% DenseNet121-0.08 & 37.3\% &67.3\% & 89.5\% \\\hline\hline
% \end{tabular}

% }
% \caption{Results on black box attack.
% }\label{tab:transfer}
% \end{table}

\begin{table}[t]
%\vspace{-4mm}
\centering
\resizebox{0.88\textwidth}{!}{
\begin{tabular}{l|lcc |lcc}
\bottomrule
Activation & Model &  $A_{rob}$ &  $A_{std}$ & Model &  $A_{rob}$ &  $A_{std}$
\\ \hline 
ReLU &ResNet18 & 5.9\%&  90.9\% & DenseNet121 & 6.6\% & 91.1\%         \\ 
\kwta &ResNet18-0.18 & 41.9\%  & 90.6\% & DenseNet121-0.18 & 26.5\% & \textbf{92.6\%} \\ 
\kwta &ResNet18-0.13 & 45.6\%  & 89.7\% &  DenseNet121-0.13 & 32.1\% & 91.7\%          \\  
\kwta &ResNet18-0.08 & \textbf{50.1\%}   & 86.1\% & DenseNet121-0.08 & 37.3\% & 89.5\% \\
% DenseNet121 (Vanilla)  & 6.6\%  & 64.8\% & 91.1\% \\ \hline
% DenseNet121-0.18 & 26.5\% &71.7\% & \textbf{92.6\%} \\\hline
% DenseNet121-0.13 & 32.1\% &70.7\% & 91.7\% \\\hline
% DenseNet121-0.08 & 37.3\% &67.3\% & 89.5\% \\\hline\hline
\toprule
\end{tabular}}
\caption{Results on black box attack.
\label{tab:transfer}}
\vspace{-5mm}
\end{table}

\begin{figure*}[t]
	\centering
	%\vspace{-1mm}
	\includegraphics[width=0.96\textwidth]{figs/loss.pdf}
	\vspace{-2mm}
	\caption{Gradient-based attack's loss landscapes in $k$-WTA \textbf{(a, b)} 
        and conventional ReLU models \textbf{(c, d)}.
            {(a,b)} \kwta Models have much more non-convex and non-smooth 
            landscapes.
	Also, the model optimized by adversarial training (b) has a lower absolute value of loss.
	}
    \label{fig:loss}
    \vspace{-4mm}
\end{figure*}

\vspace{-0.05in}
\vspace{-1mm}
\subsection{Loss Landscape in Gradient-Based Attacks}\label{sec:loss_land}
\vspace{-0.05in}
We demonstrate how $k$-WTA affect the attacker's loss landscape in gradient-based attacks.
Similar to the analysis in~\cite{tramer2017ensemble}, 
we visualize the attack loss of a model with respect to its input
on points $\bm{x}^\prime = \bm{x} + \epsilon_1 \bm{g}_1 + \epsilon_2 \bm{g}_2$,
where $\bm{x}$ is a test sample from CIFAR test set, 
$\bm{g}_1$ is the direction of the loss gradient with respect to the input,
$\bm{g}_2$ is another random direction, $\epsilon_1$ and $\epsilon_2$ 
sweep in the range of [-0.04, 0.04], with 50 samples each. 
This produces a 3D plot with 2500 data points.

As shown~in \figref{loss}, \kwta models (with $\gamma=0.1$) have a highly
non-convex and non-smooth loss landscape. Thus, the estimated gradient 
is hardly useful for adversarial searches. 
This explains why $k$-WTA models can resist effectively gradient-based attacks.
In contrast, ReLU models have a smooth loss surface, 
from which adversarial samples can be easily found using gradient descent.

Inspecting the range of loss values in \figref{loss},
%%The difference in absolute value of the loss shows that 
we find that    %%% the loss landscape of models optimized by 
adversarial training tends to 
compress the loss landscape's dynamic range
in both the gradient
direction and the other random direction, 
making the dynamic range smaller than that of the models without adversarial training.
%compare to a regular network, which is
This phenomenon has already been observed in ReLU networks~\cite{madry2017towards,tramer2017ensemble}. 
Interestingly, $k$-WTA models show a similar behavior (\figref{loss}-a,b).
Moreover, we find that in \kwta models a larger $\gamma$ 
leads to a smoother loss surface than a smaller $\gamma$ (see 
\appref{surf} for more details).

